A key to the projective model of homogeneous metric spaces

A metric introduced on a projective space yields a homogeneous metric space known as a Cayley-Klein geometry. This construction is applicable not only to Euclidean and non-Euclidean spaces but also to kinematic spaces (space-times). A convenient algebraic framework for Cayley-Klein geometries called the projective model is developed in [1, 2]. It is based on Grassmann and Clifford algebras and provides a set of algebraic tools for modeling points, lines, planes and their geometric transformations such as projections and isometries. Isometry groups and their Lie algebras find a natural and intuitive expression in the projective model. The aim of this paper is to translate the foundational concepts of the projective model from the language of projective geometry to a more familiar language of vector algebra and thereby facilitate its spread and adoption among physicists and applied mathematicians. I apply the projective model to Minkowski, de-Sitter, and anti-de-Sitter space-times in two dimensions. In particular, I show how the action of the Poincare group can be captured by the Clifford algebra in a uniform fashion with respect to rotations (boosts) and translations.

==> p-10+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-10+0_0.pdf}%
}%


==> p-10.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 170.028500pt{}%
\kern 178.058500pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-89.029250,85.014250)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-10+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -354.106298091045118781,3Droll=0,3Droo=354.106298091045118781,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-10+0.js]{175.65625pt}{167.62625pt}{\ASYprefix\jobname-10+0.prc}}


==> p-11+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-11+0_0.pdf}%
}%


==> p-11.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 171.032250pt{}%
\kern 178.058500pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-89.029250,85.516125)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-11+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -301.958881543927418534,3Droll=0,3Droo=301.958881543927418534,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-11+0.js]{175.65625pt}{168.63pt}{\ASYprefix\jobname-11+0.prc}}


==> p-12+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-12+0_0.pdf}%
}%


==> p-12.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 174.043500pt{}%
\kern 178.058500pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-89.029250,87.021750)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-12+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -358.21425875021208185,3Droll=0,3Droo=358.21425875021208185,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-12+0.js]{175.65625pt}{171.64125pt}{\ASYprefix\jobname-12+0.prc}}


==> p-13+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-13+0_0.pdf}%
}%


==> p-13.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 170.028500pt{}%
\kern 178.058500pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-89.029250,85.014250)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-13+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -366.46363057539787178,3Droll=0,3Droo=366.46363057539787178,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-13+0.js]{175.65625pt}{167.62625pt}{\ASYprefix\jobname-13+0.prc}}


==> p-14+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-14+0_0.pdf}%
}%


==> p-14.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 170.028500pt{}%
\kern 178.058500pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-89.029250,85.014250)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-14+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -310.483955999900729239,3Droll=0,3Droo=310.483955999900729239,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-14+0.js]{175.65625pt}{167.62625pt}{\ASYprefix\jobname-14+0.prc}}


==> p-15+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-15+0_0.pdf}%
}%


==> p-15.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 170.028500pt{}%
\kern 178.058500pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-89.029250,85.014250)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-15+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 0.999999999999999889,3Dcoo=0 0 -307.77410576399159936,3Droll=0,3Droo=307.77410576399159936,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-15+0.js]{175.65625pt}{167.62625pt}{\ASYprefix\jobname-15+0.prc}}


==> p-8+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-8+0_0.pdf}%
}%


==> p-8.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 170.028500pt{}%
\kern 178.058500pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-89.029250,85.014250)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-8+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -301.958881543927418534,3Droll=0,3Droo=301.958881543927418534,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-8+0.js]{175.65625pt}{167.62625pt}{\ASYprefix\jobname-8+0.prc}}


==> p-9+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-9+0_0.pdf}%
}%


==> p-9.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 170.028500pt{}%
\kern 178.058500pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-89.029250,85.014250)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-9+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 0.999999999999999889,3Dcoo=0 0 -301.958881542957612965,3Droll=0,3Droo=301.958881542957612965,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-9+0.js]{175.65625pt}{167.62625pt}{\ASYprefix\jobname-9+0.prc}}

